Two-level Dynamic Load Balancing for High Performance Scientific Applications

Scientific applications are often complex, irregular, and computationally-intensive. To accommodate the ever-increasing computational demands of scientific applications, high-performance computing (HPC) systems have become larger and more complex, offering parallelism at multiple levels (e.g., nodes, cores per node, threads per core). Scientific applications need to exploit all the available multilevel hardware parallelism to harness the available computational power. The performance of applications executing on such HPC systems may adversely be affected by load imbalance at multiple levels, caused by problem, algorithmic, and systemic characteristics. Nevertheless, most existing load balancing methods do not simultaneously address load imbalance at multiple levels. This work investigates the impact of load imbalance on the performance of three scientific applications at the thread and process levels. We jointly apply and evaluate selected dynamic loop self-scheduling (DLS) techniques to both levels. Specifically, we employ the extended LaPeSD OpenMP runtime library at the thread level and extend the DLS4LB MPI-based dynamic load balancing library at the process level. This approach is generic and applicable to any multiprocess-multithreaded computationally-intensive application (programmed using MPI and OpenMP). We conduct an exhaustive set of experiments to assess and compare six DLS techniques at the thread level and eleven at the process level. The results show that improved application performance, by up to 21%, can only be achieved by jointly addressing load imbalance at the two levels. We offer insights into the performance of the selected DLS techniques and discuss the interplay of load balancing at the thread level and process level.

==> 4.tex <==
% !TEX root =  sphynx_dlb.tex
\section{Two-level Load Balancing of Production SPH Simulations}  
\label{sec:load_balance}

%\begin{itemize}
%\item Steps of \sphynx{} application
%\item Why gravity [almost 50\% of each iteration, load imbalanced, no extra data movement is needed]
%\item Parallelization of \sphynx{}, MPI and OpenMP 
%\item Execution traces - show MPI load imbalance, show OpenMP load imbalance
%\item Load imbalance metrics, c.o.v. and mean/max
%\end{itemize}
\begin{figure*}[htbp]
	\centering
	\includegraphics[clip, trim=0cm 1.5cm 0cm 0cm, scale=0.36]{figures/trace.pdf}%
	\caption{%The \ali{two-level} load imbalance at the \tl{} and the \pl{} in \sphynx{}. The execution trace \ali{(parallelized workflow steps only, sequential workflow steps are filtered out to minimize tracing overhead)} of a single \mbox{time-step} (\mbox{time-step} 15, \ali{duration of} 8.3 seconds out of 325 seconds \ali{total execution time}) of \ali{the} Evrard collapse simulation~(\ali{c.f. Section~\ref{subsec:experiments}}) with one million particles on 10 processes and 8 threads per process on miniHPC. Particles are equally divided between the 10 processes and default (STATIC) OpenMP scheduling is used. Load imbalance at the \tl{} can be observed in the yellow regions and \pl{} load imbalance in the red regions.\\
		%Table~\ref{tbl:load_imbalance} shows the load imbalance metrics calculated for this execution.
		\ac{Impact of two-level load imbalance at \tl{} and \pl{} in \sphynx{}. The figure presents the execution trace (\ali{parallelized workflow steps only, sequential workflow steps are filtered out to minimize tracing overhead}) of \mbox{time-step} 15 of the Evrard collapse simulation~(c.f. Section~\ref{subsec:experiments}) with one million particles on 10 processes with 8 threads per process on the miniHPC system. Particles were equally divided between the 10 processes and the default (STATIC) OpenMP scheduling technique was used. Idle time due to load imbalance is shown in yellow at the \tl{} and in red at the \pl{} level.}
	}
	\label{fig:trace}
\end{figure*}

\rc{\sphynx{}\footnote{Available at http://astro.physik.unibas.ch/sphynx} is a state-of-the-art \ali{production} SPH code \cite{cabezon2017sphynx}, that is the first to include an integral approach to calculate derivatives~(IAD) and a dynamically adaptive interpolation \textit{sinc} kernel, being both elements of great importance in overcoming \mbox{long-lasting} problems of the SPH technique related \ali{to} the development of subsonic hydrodynamical instabilities \cite{cabezon2008,garcia2012}.
%that includes many recent upgrades, like adaptive interpolating \textit{sinc} kernels, an integral approach to calculate derivatives (IAD), and generalized volume elements. 
It is also one of the few hydrodynamic codes in the literature that can simulate both Type Ia and \mbox{core-collapse} Supernovas, including nuclear reactions, neutrino transport, and general relativity correction terms.
\subsection{Load Imbalance in SPHYNX}
%\sphynx{} is the first SPH code that includes an integral approach to calculate derivatives and a dynamically adaptive interpolation \textit{sinc} kernel, being both elements of great importance in overcoming long lasting problems of the SPH technique related with the development of subsonic hydrodynamical instabilities \cite{cabezon2008,garcia2012}.
The main structure of \sphynx{} is described in Algorithm~\ref{algo:sphynx}. 
After the initialization of all variables, the code proceeds to perform several time iterations (or \mbox{time-steps}), evolving the system. 
Each time iteration performs a series of \ali{computational} steps (\ali{enumerated} in Algorithm~\ref{algo:sphynx}), beginning with the creation of a tree structure used to locate neighboring particles and to calculate self-gravity. 
Then, a list of neighbors for each particle is found, \ali{this step} being central for the SPH technique. 
Once this \ali{list} is known, the SPH interpolations can be \ali{performed} to find the density distribution, the IAD terms, the thermodynamical properties of the system, and the rates of change of velocities and internal energy. 
Finally, the particles positions, velocities, and internal energy are updated, a new \mbox{time-step} is found, and a new \ali{time} iteration begins.}

%that calculate the thermodynamical properties of the system, the rates of change of capital physical properties, the gravitational force, and updates the system for the next time-step.

\begin{algorithm}[htbp]
	\small
	\caption{\sphynx{} Computational Workflow}\label{algo:sphynx}
	%initialization\\
	\For{$l\gets t_{init}$ \KwTo $t_{final}$}
	{
		1. Build tree\\
		2. Find neighbors\\
		\hspace{0.75em} 2.1 Collective communication (number of neighbors) \\
		3. Density \& grad-h calculations\\
     	\hspace{0.75em} 3.1 Collective communication (density \& grad-h)\\
		4. IAD calculations\\
      	\hspace{0.75em} 4.1 Collective communication (IAD terms)\\
	    5. EOS \& $\nabla\textbf{v}$ calculations\\
	    \hspace{0.75em} 5.1 Collective communication ($\nabla\cdot\textbf{v}$ \& $\nabla\times\textbf{v}$)\\
		6. Momentum \& energy calculations\\
     	\hspace{0.75em} 6.1 Collective communication ($\nabla P$ \& $du/dt$)\\
		7. Gravity calculations\\
	    \hspace{0.75em} 7.1 Collective communication (gravitational force and potential)\\
		8. Update velocities, position, and energy\\
		9. Time-step evaluation\\
		10. Verification via conservation laws\\
	}
\end{algorithm}

%\sphynx{} is a time-stepping application.
%The main workflow of \sphynx{} at each time-step is shown in Algorithm~\ref{algo:sphynx}. 
\sphynx{} is parallelized using MPI at the \pl{} and OpenMP \texttt{parallel for} at \ali{the \tl{}} (\ali{within each MPI rank}).
The domain (particles) is divided equally \ali{during} the initialization step among the MPI processes, and each process is assigned a \ali{chunk} of particles equals to the total number of particles $N$ divided by the number of MPI processes $P$ \ali{(straightforward decomposition)}.
\sphynx{} workflow consists of 10 main calculations \ali{interleaved with} collective communications to update the information on all the MPI processes. 
\rc{The collective communications are needed every time SPH interpolations take place, as the information of neighboring particles is \ali{required} at that moment and some neighbors might be located in a different MPI process.}

%\figurename{~\ref{fig:time_distrib}} shows the average time spent in each of the ten workflow steps per time-step in the execution of Evrard collapse and Stellar collision test-cases~(see Section~\ref{subsec:experiments}) on miniHPC\footnote{miniHPC is a fully controlled non-production HPC cluster at the Department of Mathematics and Computer Science at the University of Basel, Switzerland.} system 
%\figurename{~\ref{fig:time_distrib}} confirms that PEs spend a substantial amount of time per each time-step in gravity calculations. 

\figurename{~\ref{fig:trace}} shows the execution trace of a single \mbox{time-step} of \ali{an} Evrard collapse simulation~(\ali{c.f. Section~\ref{subsec:experiments})} with $10$ MPI processes and $8$ OpenMP threads per process on miniHPC\footnote{miniHPC is a fully controlled non-production HPC cluster at the Department of Mathematics and Computer Science at the University of Basel, Switzerland.}.
One can observe that the PEs spend a substantial amount of time per \mbox{time-step} in gravity calculations.
In fact, this pattern can be observed in most SPH simulations \ali{that include self-gravity}. 
Inspecting the execution trace reveals the load imbalance at both the \pl{} (between MPI ranks represented by the waiting time in red) and the \tl{} (between OpenMP threads represented by the waiting time in yellow).
For example, the ratio between the slowest to the fastest process finishing times for the experiment (\aliA{for the gravity calculations per \mbox{time-step})} in \figurename{~\ref{fig:trace}} is $1.4$, and 
%the difference between them is $1.18$ seconds, which means that the slowest process is loaded by nearly $50$\% more work than the fastest one
the fastest process waits for the slowest one approximately 25\% of the execution time ($1.18$s).
This load imbalance stems from the highly imbalanced \mbox{computationally-intensive} workflow steps shown in Algorithm~\ref{algo:sphynx}.
The amount of computations per particle in each of the workflow steps depends on the number of neighbors this particle has, which is irregular, and, therefore, the computational load is imbalanced.
Moreover, as the SPH simulation evolves the particles move in the physical system, changing their distribution and consequently, the number of neighbors per particle, leading to \ali{further} load imbalance.

Two metrics are considered to measure the load imbalance of the parallel execution of the applications, namely the coefficient of variation (c.o.v.) of the parallel processes finishing times~\cite{FAC} and the ratio of the mean processes finishing times to the maximum process finishing time (mean/max)~\cite{casas2008automatic}. 
The c.o.v. is calculated as the ratio between the standard deviation of processes finishing times to their mean value. 
Both metrics are unitless.
\ali{A} severe execution load imbalance corresponds to a c.o.v. $>> 0$ and a mean/max $<< 1$ \ali{while a negligible load imbalance corresponds to c.o.v. $\approx 0$ and mean/max $\approx 1$}. %a high value of c.o.v. and a low value of mean/max.

Table~\ref{tbl:load_imbalance} shows the load imbalance calculated for the \sphynx{} simulation of Evrard collapse, Stellar collision, and Stellar relaxation~(see Section~\ref{subsec:experiments} \ali{for the details describing these test-cases}) \ali{which do not employ load balancing techniques.}  
The number of ranks is chosen such that each PE is assigned at least $10,000$ particles and at most $50,000$ particles, and using $8$ threads per rank on miniHPC to avoid \ali{that} \ali{communication dominates} the execution time.
For the Stellar relaxation test-case, weak scaling is used, keeping the number of particles per PE fixed at $50,000$ \ali{and executed on the}

Piz Daint\footnote{Piz Daint is a Cray XC50 supercomputer system, the Swiss National Supercomputing Center~(CSCS), https://www.cscs.ch/computers/dismissed/piz-daint-piz-dora/.} HPC system, as it offers a large number of nodes, \ali{allowing a large number of} experiments \ali{to be executed} in parallel \ali{within a} reasonable time.
One can observe that increasing the number of processes, increases the \ali{\pl{}} load imbalance and, thus, hinders \ali{scalability}, specifically for the strong scaling executions of the first two test-cases.
\ali{For example, an increase from $4$ to $10$ processes increases} the c.o.v. from $0.07$ to $0.11$, and \ali{decreases} the mean/max value from $0.94$ to $0.89$, which indicate an increase in the load imbalance, \ali{in the case of the Evrard collapse simulation}.

\begin{table}[htbp]
	\caption{Process-level load imbalance in \ali{the} \sphynx{} simulation of Evrard collapse, Stellar collision, and Stellar relaxation with no load balancing techniques}
	\begin{center}
		\begin{adjustbox}{max width=\textwidth}
			\label{tbl:load_imbalance}
			\begin{tabular}{@{}lcc|cc|cccc@{}}
				\hline
				Test-case                                                 & \multicolumn{2}{c|}{\textbf{Evrard collapse}}                                & \multicolumn{2}{c|}{\textbf{Stellar collision}}  &  \multicolumn{4}{c}{\textbf{Stellar relaxation}}   \\ \cline{1-9}
				\begin{tabular}[c]{@{}l@{}}Number of\\ MPI ranks\end{tabular} & \multicolumn{1}{r|}{\textbf{4}} & \multicolumn{1}{r|}{\textbf{10}} & \multicolumn{1}{r|}{\textbf{14}} & \multicolumn{1}{r|}{\textbf{44}} &\multicolumn{1}{r|}{\textbf{2}} &\multicolumn{1}{r|}{\textbf{10}} &\multicolumn{1}{r|}{\textbf{20}} & \multicolumn{1}{r}{\textbf{40}} \\ \cline{1-9}
				c.o.v.  & \multicolumn{1}{r|}{$0.07$}  & \multicolumn{1}{r|}{$0.11$}  & \multicolumn{1}{r|}{$0.05$}  &  \multicolumn{1}{r|}{$0.10$} &  \multicolumn{1}{r|}{$0.03$} &   \multicolumn{1}{r|}{$0.03$} &  \multicolumn{1}{r|}{$0.03$} &   \multicolumn{1}{r}{$0.04$} \\
				mean/max  & \multicolumn{1}{r|}{$0.94$}   & \multicolumn{1}{r|}{$0.89$}   & \multicolumn{1}{r|}{$0.93$}  &  \multicolumn{1}{r|}{$0.89$}  &\multicolumn{1}{r|}{$0.97$} &   \multicolumn{1}{r|}{$0.97$} &  \multicolumn{1}{r|}{$0.97$}&   \multicolumn{1}{r}{$0.96$} \\ \hline
			\end{tabular}
		\end{adjustbox}
	\end{center}
	
\end{table}



==> 7.tex <==
\section{Existing Reproducibility Efforts}
\label{sec:repefforts}

Many efforts have been carried out to reproduce results from computer science research.  However, reproducing other researchers' experiments is not an easy task. According to the study carried out by Collberg and his team in University of Arizona, USA \cite{repcollberg}, they were able to reproduce only $24.9\%$ out of 613 papers downloaded from eight different ACM conferences. Even more, their reproducibility process was not always straightforward, as in some cases they had to search for the code, had many difficulties during the build process, and needed to contact the authors to ask for more information.\\

Another interesting reproducibility study was performed by Carpen-Amarie et al. \cite{repcarpen}. The authors focused on a smaller set of papers compared to the previous study, as only papers published in the proceedings of the 2013 EuroMPI conference were considered. Two main phases for reproducibility were defined: data acquisition phase and data analysis phase. Data acquisition phase involves source code availability, dependencies declaration, environment configuration, build process configuration, input data, and a description of how to execute the code in the same settings as the original experiment. On the other hand, the data analysis phase includes acquiring the output data and data processing to reach the results presented in the original publication. Papers under study were classified based on their degree of reproducibility and the top two papers after classification were chosen to reproduce them. Even though the source code and input data were available, it was needed to contact the authors for further assistance with setting up the experiment environment and had to manually modify the execution scripts to match their system configuration.\\

In 2014, Guerrera et al. experimented with reproducing the stencil wave equation using five different methods and toolsets from the literature \cite{guerrera}. Three main elements of the experiment were identified: the problem, the method, and the computing system. A micro-experiment was defined as when one tries to redo the original experiment changing only one element of the three main elements of the experiment, whereas a macro-experiment was defined as a set of micro-experiments where one element was changed while maintaining the other two elements. They have also introduced a workflow to perform reproducible computer science experiments.\\

Although there are few efforts in reproducing computer science experiments, to the best of our knowledge, there is no published work that tried to reproduce scheduling experiments in simulation or by native execution and verify their performance.



